Toward the Automated Localization of Buggy Mobile App UIs from Bug Descriptions

Bug report management is a costly software maintenance process comprised of several challenging tasks. Given the UI-driven nature of mobile apps, bugs typically manifest through the UI, hence the identification of buggy UI screens and UI components (Buggy UI Localization) is important to localizing the buggy behavior and eventually fixing it. However, this task is challenging as developers must reason about bug descriptions (which are often low-quality), and the visual or code-based representations of UI screens. This paper is the first to investigate the feasibility of automating the task of Buggy UI Localization through a comprehensive study that evaluates the capabilities of one textual and two multi-modal deep learning (DL) techniques and one textual unsupervised technique. We evaluate such techniques at two levels of granularity, Buggy UI Screen and UI Component localization. Our results illustrate the individual strengths of models that make use of different representations, wherein models that incorporate visual information perform better for UI screen localization, and models that operate on textual screen information perform better for UI component localization -- highlighting the need for a localization approach that blends the benefits of both types of techniques. Furthermore, we study whether Buggy UI Localization can improve traditional buggy code localization, and find that incorporating localized buggy UIs leads to improvements of 9%-12% in Hits@10.

==> introduction_ase_23.tex <==

\section{Introduction}
\label{sec:intro}

Bug report management is an essential, yet costly process in software maintenance \cite{zou2018practitioners}. It requires high developer effort~\cite{zou2018practitioners,Zimmermann2010,Anvik2006,fan2018chaff,Bissyande2013,Tian2015a} due in part to the potential for large volumes of reported bugs and the varying quality of submitted reports. Submitted reports are the central artifact in bug management~\cite{Zimmermann2010,zou2018practitioners,fan2018chaff,Chaparro2017-2}, as they directly impact various downstream tasks such as bug triaging, reproduction, fault localization, and program repair. Bug reports typically consist of textual descriptions of defects found during software usage and testing, which are expected to include, \textit{at minimum}, the system's observed (incorrect) behavior (\textbf{OB}), the expected behavior (\textbf{EB}), and the steps to reproduce the bug (\textbf{S2Rs})~\cite{Bettenburg2008a,Laukkanen2011,Zimmermann2010,Chaparro2017-2,soltani2020significance,song2020bee}.



\looseness=-1

However, the various software maintenance tasks that comprise bug report management can vary across software domains. For instance, prior studies have shown that, for user-facing software, nearly half of the code of a given application is typically directly related to the user interface~\cite{myers1992survey}. As such, for GUI-centric software domains, such as mobile platforms, a fundamental task in the bug management process is to identify the UI screens and components (\eg buttons or text fields) that cause and/or show the incorrect behavior of the software (\ie the OB), which is necessary to understand, diagnose, and resolve the underlying bugs. This task can be difficult for developers, especially for cases when the bug reports fail to include important details and/or graphical information (\eg buggy app screenshots~\cite{erfani2014works}, and developers are subject to other mobile development constraints such as rapidly evolving platform APIs~\cite{Linares2013} and the need to support fragmented device ecosystems~\cite{Wei:ASE16}. Despite its importance, prior work has not explored the possibility of assisting developers in this task -- despite the growing body of research on automating other bug report management tasks~\cite{he2020duplicate,akbar2020large,lee2018bench4bl,Ye2016b,Moreno2014,ciborowska2022fast,Wong2014,Kochhar2014,florez2021combining,chaparro2019using,Chaparro2017-3,Zhou2012a,chaparro2019reformulating,Zhao2019,wu2021data,zhao2022recdroid+,su2022constructing}.

\looseness=-1

In this context, we argue that an automated approach that can accurately map or trace a bug description (\aka an OB description) to relevant UI screens and components is needed (we will refer to the problem as {\textbf{\textit{OB-UI Mapping}}}), not only to assist developers during bug triage and resolution but also to help improve the effectiveness of existing techniques that automate bug report management tasks~\cite{Zhao2019,zhao2022recdroid+,Fazzini2018,song_toward_2022,Chaparro:FSE19,song_burt_2023}. For example, techniques that leverage the S2Rs to automatically reproduce the reported bugs~\cite{Zhao2019,zhao2022recdroid+} or generate test cases~\cite{Fazzini2018} can benefit from an OB-UI mapping approach that suggests buggy UI screens, as these could be used to generate assertions that verify if the reported bugs can be replicated. Additionally, an OB-UI mapping approach can help existing techniques verify the quality of OB descriptions more accurately~\cite{song_toward_2022,Chaparro:FSE19,song_burt_2023}, by checking how well the description maps or links to UI screens/components, thus providing potentially better guidance to reporters about their bug descriptions and collecting higher-quality OB information in bug reports. An OB-UI mapping approach can also be useful in enhancing textual bug reports with UI screenshots so that it can assist developers in comprehending and resolving software issues more effectively \cite{nayebi2020eye,yusop2016reporting,agrawal2022understanding,Breu2010,Zimmermann2010}. This can further benefit existing techniques that detect duplicate bug reports using visual information \cite{Wang:IST19}. 

OB-UI mapping can be framed as a retrieval task and accomplished in at least two possible ways: text-to-image mapping and text-to-text mapping. More specifically, to define this task, we assume the use of an automated input generation tool~\cite{Moran2016,mao2016sapienz,choudhary2015automated,li2017droidbot,ORBITYang,machiry2013dynodroid,Gu:ICSE'19,Su:FSE'17}, the existence of test cases, or the use of beta testers that can generate screenshots and UI metadata that form a corpus of screen data for a given application. 
The goal of this paper is to explore the capabilities of existing textual and multi-modal (visual-textual) deep learning (DL) techniques for automatic OB-UI mapping. The study focuses on two retrieval tasks for the OB-UI mapping problem: \textbf{\textit{screen retrieval (SR)}}, which involves retrieving UI screens that most likely correspond to a given bug description, and \textbf{\textit{component retrieval (CR)}}, which aims to retrieve UI components from a given screen relevant to the bug description.
\looseness=-1






Our study examines three DL models: a supervised text-based model (\sentbert or  \sbert~\cite{reimers2019sentence}), and two supervised textual-visual learning models (\clip~\cite{radford2021learning} and \blip~\cite{li2022blip}). We have made necessary adjustments and conducted extensive experiments on these models as they are not tailored to solve our problem. The main challenge of using these models for our task is the lack of an existing OB-UI dataset. To overcome this we created two novel datasets: a \textit{synthetic dataset}, and a \textit{real dataset}. We fine-tuned the DL models using the \textit{synthetic dataset} and evaluated the effectiveness of the models in zero-shot and fine-tuned settings using the two novel datasets. The \textit{synthetic dataset} includes 2.8M OB descriptions automatically created for 23.9k mobile app UI screens, via textual templates designed/implemented for a variety of mobile app bug types. The \textit{real dataset} includes 127 OB descriptions and associated UI screens/components, manually tagged in 53 real bug reports from the AndroR2 dataset~\cite{wendland2021andror2}. The two datasets include two types of bug descriptions: \textit{screen OBs}, which describe a bug that affects an entire UI screen, and \textit{component OBs}, which describe a bug that affects specific UI components of a screen.



Our results reveal that no single technique universally performs best across all OB types and retrieval tasks. The best-performing approaches (\blip and fine-tuned \sbert) can suggest correct UI screens and components in the top-3 recommendations for 53\% and 70\% of the bug descriptions, respectively. The study also found that fine-tuning, based on the synthetic dataset, is more effective for component retrieval than for screen retrieval, and the models tend to perform better for higher-quality bug descriptions.




Our study has several implications for bug report management research. First, despite the studied techniques being effective for OB-UI mapping, there is still room for improvement. Second, a specialized OB-UI mapping technique should blend the benefits of both textual and multimodal-based techniques. Third, it is key to consider different types of bug descriptions and their quality levels when designing OB-UI mapping techniques. Finally, large-scale real datasets for OB-UI mapping are necessary to achieve higher retrieval performance.

\noindent In summary, this paper makes the following contributions:
\begin{enumerate}
	\item A novel synthetic dataset of OB descriptions and associated UI screens/components that can be utilized for pre-training/fine-tuning OB-UI mapping techniques.
	\item A novel dataset of real-life OB descriptions and associated UI screens/components that can be utilized for evaluating OB-UI mapping techniques.
	\item A comprehensive empirical study that evaluates the effectiveness of three  DL techniques of different kinds, used for OB-UI mapping. The study reveals different performances achieved by the approaches for different types of OBs and retrieval tasks.
	\item A complete replication package that provides data, source code, results, and instructions to reproduce the study \cite{package}.
\end{enumerate}


==> introduction_old.tex <==

\section{Introduction}
\label{sec:intro}

\os{TODO}\kevin{TODO} Bug report management is an essential, yet costly process in software engineering~\cite{zou2018practitioners}. Software projects typically receive a significant number of bug reports on a daily basis, demanding a high effort from developers as they require to understand, prioritize, assign, replicate, localize, and fix the reported bugs~\cite{zou2018practitioners,Zimmermann2010,Anvik2006,fan2018chaff,bissyande2013got}. Given the importance of this process, researchers have proposed a variety of techniques to automate these tasks~\cite{zou2018practitioners}, aiming to reduce developers' effort and improve their effectiveness.

Essential to existing bug management techniques are bug reports~\cite{Zimmermann2010,zou2018practitioners,fan2018chaff}: textual descriptions of defects found during software usage and testing. Bug reports are meant to include the necessary information for developers to carry out the bug management process, describing at minimum, the system's observed (\aka unexpected) behavior (\textbf{OB}), the expected behavior (\textbf{EB}), and the steps to reproduce the bug (\textbf{S2Rs})~\cite{Bettenburg2008a,Laukkanen2011,Zimmermann2010,Chaparro2017-2,soltani2020significance}.
\looseness=-1

Existing techniques that automate bug management tasks typically leverage entire textual descriptions or specific parts of bug reports~\cite{Chaparro:FSE17}\re, tracing or mapping this information to relevant software artifacts \re, such as source code \cite{Moreno2014}\re, other bug reports \cite{imran2021automatically}\re, code change sets \re, screenshots of the software's user interface (UI) \re, and UI metadata \re. For example, researchers have leveraged combinations of OB, EB, and S2R descriptions to trace and retrieve duplicate bug reports~\cite{chaparro2019reformulating} and buggy source code via IR-based techniques~\cite{florez2021combining,chaparro2019using,Chaparro2017-3}.
\looseness=-1



\os{rephrase these next two paragraph}
In recent years, a growing body of research in the software engineering community has focused on mapping or linking bug report descriptions to graphical artifacts of mobile apps such as screenshots that depict the app's graphical user interface (GUI), to address various bug management tasks~\cite{Zhao2019,zhao2022recdroid+,Fazzini2018,song_toward_2022,Chaparro:FSE19,song_burt_2023} \re. For example, researchers have leveraged the S2Rs in bug reports to automatically reproduce the reported bugs~\cite{Zhao2019,zhao2022recdroid+} or to generate test cases~\cite{Fazzini2018}, by associating individual S2Rs to UI metadata and images via textual matching. Other researchers have focused on assessing the quality of EB and S2R descriptions and giving feedback to reporters about missing or inaccurate information~\cite{song_toward_2022,Chaparro:FSE19,song_burt_2023}, by mapping these descriptions to UI screens and metadata via heuristics and text-matching techniques. Likewise, other research has focused on generating commands from textual UI actions (\eg described in test reports) by utilizing visual and multi-modal learning models that automatically process UI screens and metadata~\cite{}\re.

One important challenge that prior research has not adequately addressed is accurately mapping OB descriptions (\aka bug descriptions) to relevant app UI screens and components, which is essential to automate various bug report management tasks. For example, existing bug reproduction and test case generation techniques~\cite{Zhao2019,zhao2022recdroid+,Fazzini2018} are successful in generating executable commands that replicate the reported S2Rs but are unable to generate test assertions from OB (and EB) descriptions that can be used to verify if the bug is replicated. Similarly, existing techniques that verify OB quality rely on heuristics and basic text-matching approaches that often fail to associate OB descriptions and corresponding UI screens/metadata~\cite{song_toward_2022,Chaparro:FSE19,song_burt_2023}, potentially giving misguidance to reporters or failing to collect high-quality OB information in bug reports. Mapping OB descriptions to UI screens and components can not only serve to automate these tasks but also augment textual bug reports with graphical information, which can help developers better understand and address software problems~\cite{nayebi2020eye,yusop2016reporting,agrawal2022understanding,Breu2010,Zimmermann2010}, and enable the benefits of other bug management techniques (\eg duplicate bug report detection~\cite{Wang:IST19}).

To address this challenge, this paper reports the first comprehensive study that evaluates the capabilities of textual and visual-textual information retrieval (IR) and deep learning (DL) techniques in automatically mapping OB descriptions to relevant app UI screens and components. The study focused on two retrieval tasks for the OB-UI mapping problem: \textit{screen retrieval}, which involves retrieving UI screens that most likely correspond to a given bug description, and \textit{component retrieval}, which aims to retrieve UI components from a given screen that most likely correspond to the bug description.

The study evaluated four retrieval techniques: a basic unsupervised text-based IR technique (\lucene~\cite{Hatcher2004}), a supervised text-based DL model (\sentbert \re), a supervised visual-text contrastive DL model (\clip \re), and a supervised visual-text contrastive/captioning-filtering DL model (\blip \re), tailored for two retrieval tasks.

We evaluated the techniques in zero-shot and fine-tuned settings, using two novel datasets: a \textit{synthetic}, large-scale dataset for fine-tuning the DL models and a \textit{real dataset} for assessing technique effectiveness. \os{to update the numbers} The \textit{synthetic dataset} comprises XX OB descriptions of XX mobile app UI screens and was generated automatically via textual templates designed/implemented for a variety of mobile app bug types. The \textit{real dataset} comprises XX OB descriptions manually tagged in XX real-life bug reports from the AndroR2 dataset~\cite{wendland2021andror2} and associated UI screens/components. \os{Say that these OBs have different quality levels and describe different bug types.} The two new datasets include two types of bug descriptions: \textit{screen OBs}, which describe a bug that affects an entire UI screen, and \textit{component OBs}, which describe a bug that affects one or more UI components of a screen.

\os{Add numerical results}
The study results reveal that no single technique universally performs best across all OB types and retrieval tasks. Instead, for the screen retrieval task, the two textual-based techniques perform better when using component OBs and the two multi-modal techniques perform better when using screen OBs as input. For the component retrieval task, the two textual-based techniques perform better than the multi-modal techniques. \os{remove this} The study also found that model fine-tuning does not necessarily lead to better retrieval performance, indicating that pre-training using general-purpose large-scale data is beneficial for OB-UI mapping. We discuss the potential reasons for these results and propose different directions of future work.

Our study has implications for bug report management research. First, a comprehensive OB-UI mapping technique should blend the benefits of both textual-based and multimodal-based techniques. Second, it is key to consider different types of bug descriptions when designing OB-UI mapping techniques. Finally, large-scale real datasets for OB-UI mapping are necessary to achieve higher retrieval performance.

In summary, this paper makes the following contributions:
\begin{enumerate}
	\item A novel synthetic dataset of OB descriptions and associated UI screens/components that can be utilized for pre-training/fine-tuning OB-UI mapping techniques.
	\item A novel dataset of real-life OB descriptions and associated UI screens/components that can be utilized for evaluating OB-UI mapping techniques.
	\item A comprehensive empirical study that evaluates the effectiveness of four IR/DL retrieval approaches, used for OB-UI mapping. The study reveals different performances achieved by the approaches for different types of OBs and retrieval tasks and propose various directions of future work.
	\item A complete replication package that provides data, source code, results, and instructions to verify and reproduce the study \re.
\end{enumerate}

In the remaining of this paper, we use observed behavior (OB) and bug descriptions interchangeably.


==> results_old.tex <==

\begin{table}[t]\centering
	\caption{Screen/component retrieval results on synthetic~data} 
	\label{tab:synthetic_results}
	\setlength{\tabcolsep}{3pt}
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccccl|cccll}
	\toprule
	\multirow{2}{*}{\textbf{Approach}} & \multicolumn{5}{c|}{\textbf{Screen Retrieval}} & \multicolumn{5}{c}{\textbf{Component Retrieval}} \\ \cline{2-11} 
	& \multicolumn{1}{c|}{\textbf{MRR}} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \multicolumn{1}{c|}{\textbf{MRR}} & \textbf{H@1} & \textbf{H@2} & \multicolumn{1}{c}{\textbf{H@3}} & \textbf{H@4} \\ \hline
	\sbert & \multicolumn{1}{c|}{0.538} &	0.355 &	0.526 &	0.642 &	0.726 & \multicolumn{1}{c|}{0.610}	& 0.482 & 	0.599 & 	0.671 & 	0.725 \\
	\sbertf & \multicolumn{1}{c|}{0.590} &	0.418 &	0.587 &	0.699 &	0.774  & \multicolumn{1}{c|}{0.747}	& 0.667 & 	0.740 & 	0.783 & 	0.818  \\ \hline
	\clip & \multicolumn{1}{c|}{0.492} & 0.304  & 0.470 & 0.591 &  0.679 & \multicolumn{1}{c|}{0.474} &  0.334  & 0.449  & 0.522 & 0.582   \\
	\clipf & \multicolumn{1}{c|}{0.619} & 0.453 & 0.626 & 0.730 & 0.798 & \multicolumn{1}{c|}{0.704} & 0.605 &0.701   & 0.754   &  0.793 \\ \hline
	\blip & \multicolumn{1}{c|}{0.543} & 0.373 & 0.530 & 0.633 &  0.709& \multicolumn{1}{c|}{0.436} & 0.253 & 0.376 & 0.563 & 0.629 \\
	\blipf & \multicolumn{1}{c|}{0.628} & 0.475  & 0.634 & 0.724 & 0.788 & \multicolumn{1}{c|}{0.698} &  0.612& 0.688 & 0.733 & 0.768 \\ \bottomrule
	\end{tabular}%
}
\vspace{-0.5cm}
\end{table}




\section{Results Analysis and Discussion}
\label{sec:results}

We present and discuss the effectiveness results of the approaches for both screen (SR) and component retrieval (CR). We focus our discussion on the MRR results, since the other metrics show similar trends to the MRR results, for the best model training configurations. Our replication package contains the results of all the experiments we conducted \cite{package}.

\Cref{tab:synthetic_results} shows that the fined-tuned models outperform their zero-shot counterparts for both retrieval tasks on the synthetic test set (by 9.6\% - 25.8\% MRR), indicating the models learned from synthetic textual and/or visual UI information. \clipf achieves the highest improvement over its zero-shot model, followed by \blipf, and \sbertf. Overall, \blipf is the most performing model among all. 

\subsection{\ref{rq:screen_retr}: Screen Retrieval Results}
\label{sec:screen_retr_results}


\Cref{tab:screen_retr_results} show the screen retrieval performance of the approaches for the 228 queries. The results reveal that \blip performs the highest (0.457 MRR), beating the second best \sbert (0.415 MRR) and the third best \lucene (.411 MRR) with a relative improvement of 10.1\% \& 11.31\% respectively. While \lucene performs similarly to \sbertf and beats the other four models with a smaller margin, it fails to retrieve screens in 18 cases (not shown in the table). However, \lucene achieves competitive H@1 like the best model \blip (.285). 

The results indicate the models, particularly \blip and \sbert, are effective for screen retrieval, which means their rich representations, learned from images and text from other domains, can be transferred to OB-UI mapping. This implies that both sources of information (UI pixels and text) are beneficial for the task. Interestingly, although \sbert only leverages textual information which makes it potentially less expensive to train/execute, it can secure the second spot.





The results also indicate that there is still room for improvement, as the best model (\blip) can suggest the expected UI screens in the top-1 to top-3 recommendations in about 29\% to 52\% of the cases (see the H@1-3 results in \cref{tab:screen_retr_results}). Additionally, as the results show, fine-tuning affects the models' performance. It is important to note that the fine-tuning of \blip was done with text-image pairs containing duplicate images across pairs (since there are multiple OBs per UI screen). We attempted to train \blip with the same unique text-image dataset used for \clip, consisting of 14.3k pairs. This was motivated mainly by the \blip's contrastive/matching losses, which might benefit from the unique dataset. However, \blip was not able to learn from this dataset as we did not observe a steady, decreasing training loss. We attribute this to the relatively low size of this dataset. Since \blip is a larger model than \clip (224M vs 151M parameters), given its more robust architecture, it needs more data for training. 



Finally, we found a small-to-moderate positive correlation between the OB quality ratings and the MRR results: we obtained a Spearman's correlation of 0.1  to  1.0 across models all except \clip. This generally indicates that higher OB quality leads to higher retrieval performance.




\begin{table}[t]\centering
\centering
\caption{Screen retrieval results on real data}
\label{tab:screen_retr_results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Approach} & \textbf{MRR} & \textbf{MAP} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
BLIP\_zs  & 0.457 & 0.443 & 0.285 & 0.447 & 0.518 & 0.592 & 0.671 \\ \hline
SBERT\_zs & 0.415 & 0.385 & 0.259 & 0.390 & 0.456 & 0.526 & 0.557 \\ \hline
LUCENE    & 0.411 & 0.384 & 0.285 & 0.386 & 0.465 & 0.522 & 0.575 \\ \hline
BLIP\_ft  & 0.393 & 0.381 & 0.241 & 0.355 & 0.417 & 0.500 & 0.557 \\ \hline
CLIP\_zs  & 0.381 & 0.348 & 0.206 & 0.338 & 0.465 & 0.526 & 0.592 \\ \hline
SBERT\_ft & 0.381 & 0.360 & 0.224 & 0.355 & 0.447 & 0.491 & 0.518 \\ \hline
CLIP\_ft  & 0.380 & 0.353 & 0.232 & 0.316 & 0.412 & 0.461 & 0.553 \\ \hline
\end{tabular}%
}
\end{table}
















\subsection{\ref{rq:component_retr}: Component Retrieval Results}
\label{sec:component_retr_results}
\Cref{tab:component_retr_results} show the component retrieval results of all the approaches for 254 retrieval tasks. Note that although the \# of OB is 228, some OBs may have a different component corpus for retrieval, one for each screen in the ground truth (\ie one OB/bug description may correspond to multiple buggy UI screens).
The results reveal that all DL approaches (except \clipf) perform higher (0.413+ MRR) than the baseline (\lucene), which achieves 0.398 MRR. Even if \lucene achieves a slightly higher MRR than \clipf (.392 MRR), it fails to retrieve UI component suggestions in 66 cases out of 254 tasks. 

\sbert is the most effective of all approaches (0.517 MRR) and outperforms the second best model (\blipf) and the sixth best model (\lucene) with a relative improvement of 4.93\% \& 29.7\% respectively. This model can suggest the expected UI component in the top-1 to top-3 results in about 34\% to 60\% of the cases. Among all the fine-tuned models, \blipf achieves the highest performance (.492 MRR) surpassing the second performing fine-tuned model \sbertf (.413) by 19.13\% relative improvement. Important to note that \blipf beats \blip (.424 MRR) with a relative improvement of 16.04\%.


Several observations can be derived from these results. First, the superiority of \blipf compared to \blip suggests that the models can learn from the synthetic OB/bug descriptions and their corresponding UI components. Second, there is still room for improving automated OB-UI mapping. While the mapping performance of the best model is not low, the performance is not very high either. Specialized models for OB-UI component retrieval are needed. Third, the textual information present in the UI components of the screens seems to be highly effective in performing OB-UI mapping, as indicated by \sbert and \sbertf's results. Fourth, \blip/\blipf superiority over \clip/\clipf seems to stem from architectural differences, as \blip is specifically designed for text-image matching (via two losses: contrastive and matching), unlike \clip, which aims to learn joint representation for text and images via contrastive learning without an explicit matching loss. Fifth, while it may be counter-intuitive that \sbert outperforms the multi-modal approaches, we generally observed that OBs tend to describe the buggy components using a language that is more similar to the component text observed by the user, which a language model like \sbert is specifically designed for. While \blip also leverages textual information of the components, it does so based on the pixel data mainly, rather than the actual component text extracted from the UI metadata. 


\begin{table}[h]\centering
\centering
\caption{Component retrieval results on real data}
\label{tab:component_retr_results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Approach} & \textbf{MRR} & \textbf{MAP} & \textbf{H@1} & \textbf{H@2} & \textbf{H@3} & \textbf{H@4} & \textbf{H@5} \\ \hline
SBERT\_zs & 0.517 & 0.504 & 0.339 & 0.512 & 0.598 & 0.701 & 0.744 \\ \hline
BLIP\_ft  & 0.492 & 0.466 & 0.335 & 0.457 & 0.547 & 0.638 & 0.709 \\ \hline
BLIP\_zs  & 0.424 & 0.405 & 0.244 & 0.417 & 0.500 & 0.567 & 0.614 \\ \hline
SBERT\_ft & 0.413 & 0.406 & 0.248 & 0.394 & 0.496 & 0.547 & 0.594 \\ \hline
CLIP\_zs  & 0.413 & 0.399 & 0.244 & 0.386 & 0.472 & 0.567 & 0.618 \\ \hline
LUCENE    & 0.398 & 0.355 & 0.311 & 0.441 & 0.480 & 0.504 & 0.512 \\ \hline
CLIP\_ft  & 0.392 & 0.372 & 0.224 & 0.370 & 0.476 & 0.516 & 0.571 \\ \hline
\end{tabular}%
}
\end{table}


















\subsection{\ref{rq:query_quality}: Performance of SR \& CR for different query quality and retrieval difficulty levels}



\subsection{\ref{rq:bl_experiments}: Bug Localization with SR Results}
\label{sec:bl_results}
\antu{Describe the results of the RQs of the BL study}
Table X \antu{Update the table and the ref} presents the automatic BL results of the best configurations and the baselines. Note that we conducted experiments on all the feasible manual BL configurations proposed by \re and we observed that several configurations outperform the baselines for both LUCENE and BugLocator with all the mapping settings (\ie concatenated OB, title OB, \# of screens 3 and 4).

In automatic BL, for both models, the best BL configuration is filtering with GUI Screen Components (SC)and boosting with GUI Screen (GS) with no query expansion. Note that this configuration is also best for manual BL shown by \re. For BugLocator, both SR approach of OB-UI mapping (\ie concatenated OB and first OB) leads to the best BL performance improving the baseline by 11.13\% in terms of Hit@10. On the other hand, for LUCENE, the first OB approach of SR provides the best performance beating the baseline with a relative improvement of 8.21\% for Hit@10. We also compared the automatic BL results with the manual BL results. Not surprisingly, the performance of the manual BL is slightly better than the automatic BL as the OB-UI mapping results are not perfect. We conclude that this small deterioration in the performance is not a big deal considering OB-UI mapping can automate the BL process completely. 

From the results, it is clear that the OB-UI mapping task can be used in GUI information-based bug localization and it can eliminate the manual labor of collecting the interaction traces completely. In other words, OB-UI mapping can fully automate the GUI information-based bug localization process while achieving a competitive performance.

\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/BL_Results.png}
    \caption{Best Performing Configurations of BL Experiments}
    \label{fig:enter-label}
\end{figure}




\subsection{Discussion}
\label{sec:results_discussion}

\textbf{SR \textit{vs} CR}. We found performance differences between SR (0.351 - 0.438 MRR) and CR (0.395 - 0.587 MRR), even for the zero-shot models. Several factors make SR more challenging than CR. First, the corpus size is larger and the ground truth is smaller for SR than for CR. Secondly, screen OBs are more abstract or general than component OBs in many cases. Third, the quality of the OBs matters. For instance, \textit{``Modify account B, crash occurred"} is a screen OB with a rating of 4. The best model \blip identified the relevant screen for this bug at 17th place. We observed lower-quality real screen OBs than component OBs, which seems to affect model performance.



\textbf{Zero-shot \textit{vs} fine-tuned models.} Although fine-tuned models achieved a better performance than their zero-shot models for CR, this scenario did not happen for SR. The primary reason behind this lies in the training dataset, as it mainly contains component OBs with few screen OBs, which makes the models not adequately learn the relationships between screen OBs and images for SR. Conversely, the component OBs are effective for CR. While is it more challenging to generate synthetic screen OBs, by design we generated screen OBs for selected UI screens to prevent the models from not being able to distinguish between different OBs/images. Our future work will experiment with additional screen OBs.



\textbf{Textual \textit{vs} multi-modal models.} Our study found that the \sbert is effective for OB-UI mapping (while not being the best for CR). This means textual information from UI metadata alone is useful for OB-UI mapping. On the other hand, it is difficult to identify  patterns between (screen) OB and UI images, affecting the performance of the multi-modal approaches. One potential reason is that pixel information may not be enough to detect textual patterns from the images.  Leveraging UI textual metadata directly, rather than from images, might be required to improve model performance.



\textbf{Design requirements for OB-UI mapping approaches.} The results suggest that both textual and visual information are helpful for OB-UI retrieval and fine-tuning may not be enough to achieve good retrieval performance, at least for SR. Specialized models may be required for specific OB-UI retrieval tasks, which blend the benefits of textual and visual information. Other sources that can be explored are UI hierarchy information, which has shown promising results for command/instruction UI grounding~\cite{ li2020mapping, li2021vut}. Moreover, for a successful OB-UI mapping approach, we may require a potentially distinct and diverse training dataset for SR \& CR.







==> study_design_old.tex <==



\section{Study Methodology}
\label{sec:methodology}

This study aims to investigate different methods for automatically mapping bug/OB descriptions and app UI screens/components and measure their effectiveness for this problem. 

To that end, we investigate existing retrieval approaches that leverage textual and/or visual information from the bug descriptions and UI screen/components, to perform screen and component retrieval.  With this in mind, we formulate two research questions (RQs):

\begin{enumerate}[label=\textbf{RQ$_\arabic*$:}, ref=\textbf{RQ$_\arabic*$}, itemindent=0cm,leftmargin=1cm]
    \item \label{rq:screen_retr}{\textit{How effective are retrieval approaches at mapping bug descriptions and UI screens (SR)?}}
    \item \label{rq:component_retr}{\textit{How effective are retrieval approaches at mapping bug descriptions and UI components (CR)?}}
    \item \label{rq:query_quality}{\textit{What is the performance of the retrieval approaches for both SR \& CR for different query quality and retrieval difficulty levels?}}
    \item \label{rq:bl_experiments}{\textit{How effective is the best screen retrieval approach for automating bug localization?}}
\end{enumerate}

To answer the RQ1 \& RQ2, we selected three supervised approaches of various kinds (\cref{subsec:approaches}). Then, we constructed a synthetic dataset for fine-tuning the approaches (\cref{subsec:synthetic_data}), as well as a real-life dataset for evaluating the effectiveness of the approaches (\cref{subsec:real_data}). We evaluated the approaches in zero-shot and fine-tuned settings, experimenting with different training procedures and data (\cref{subsec:eval_settings}) and measuring their performance with standard retrieval metrics (\cref{subsec:metrics}). To answer RQ3, we utilized the retrieved screens by the best screen retrieval approach to fully automate a SOTA bug localization approach \re (\cref{subsec:bl_methodology}).
\looseness=-1


\subsection{Retrieval Approaches}
\label{subsec:approaches}







We investigated three state-of-the-art deep learning (DL)-based approaches that support text-to-text or text-to-image retrieval for accomplishing OB-UI mapping tasks.

\textbf{\sentbert} (or \textbf{\sbert})~\cite{reimers2019sentence} is a neural text-based language model, derived from a pre-trained model, \bert~\cite{devlin2018bert}. \sbert receives a textual description and outputs an embedding that can be compared with an embedding of another description to establish their semantic similarity. \sbert augments the traditional \bert model with siamese and triplet networks allowing for better support of tasks such as clustering and semantic search with less computational overhead. 
\sbert can be utilized for SR/CR using the textual information in the bug description and UI screens/components.


 
\textbf{\clip}~\cite{radford2021learning} is a neural multi-modal vision/language model that can learn semantic embeddings from text and images, via a contrastive architecture. Given a pair of text-image, \clip is able to determine the similarity of the text to refer to the image, hence it can be used for text-image or image-text retrieval. 
\clip was trained on a wide range of open-source text-image datasets for a variety of domains and has been evaluated on multiple downstream tasks under zero-shot settings, achieving similar performance as ResNet-50 \cite{he2016deep} (\eg on ImageNet \cite{deng2009imagenet}). \clip can be utilized for SR/CR using textual information from the bug description and visual information from UI screens/components.







\textbf{\blip}~\cite{li2022blip} is a neural multi-modal model for  vision-language understanding and generation tasks. It utilizes a multi-modal encoder-decoder component (MED) and a captioning-filtering (CapFilt) component, incorporating three types of losses to learn representations from text and images: contrastive, matching, and language modeling losses. \blip's CapFilt improves the quality of training examples by generating synthetic labels for a given image and by filtering noisy generated image-text pairs. \blip exhibited state-of-the-art performance on image-text retrieval, image captioning, and question-answering tasks. We used a \blip version optimized for text-image retrieval tasks, which implements the multi-modal contrastive and matching losses only.  \blip can be utilized the same way \clip is used for SR and CR.
\looseness=-1

While these models have been pre-trained with general-purpose data (\eg images of landscapes and corresponding captions/descriptions), they have been shown to perform well under zero-shot settings~\cite{reimers2019sentence,li2022blip,radford2021learning} and also have been fine-tuned for diverse tasks~\cite{zhang2022pointclip,baldrati2022conditioned,conde2021clip,rasheed2022fine}. This means they can learn rich visual and textual representations that can be transferred to solving a diverse set of problems. 

Besides these three, we considered models specifically designed for mobile app UI understanding tasks, including \uibert~\cite{bai2021uibert}, \vut~\cite{li2021vut}, and \stov~\cite{li2021screen2vec}. However, \uibert and \vut's source code and pre-trained models are not available. \stov would require a significant adaptation effort for our task as the model is only designed for  generating UI screen embeddings from screen text and UI hierarchies and  extra modules would be required to adapt this model for OB-UI retrieval. We should note, though, that we experimented with it as a zero-shot encoder to represent UIs and with an \sbert model for representing bug descriptions, computing the cosine similarity on both embeddings to establish similarity. Unfortunately, this led to poor performance for both CR and SR, hence we decided to not report their performance in this paper. Our replication package contains those results~\cite{package}. 



Finally, we selected \textbf{\lucene}~\cite{Hatcher2004} as a baseline technique for text retrieval.  \lucene is an unsupervised approach that combines the classical vector space model (VSM), based on the TF-IDF representation, and the boolean text retrieval model, to compute the (cosine) similarity between a query and a document. \lucene can be utilized for SR/CR using the textual information in bug descriptions and UI screens/components.








\subsection{Synthetic Dataset Construction}
\label{subsec:synthetic_data}
















We built a synthetic dataset of bug descriptions and associated UI screens/components to fine-tune the selected DL models, given that no dataset exists for the OB-UI mapping problem. We opted to create a synthetic dataset because the models require large amounts of training data, and it would be extremely expensive to build it manually (\eg manual issue analysis).
\looseness=-1


To build our dataset, we leveraged the \ricosca dataset by Wang \etal~\cite{Wang:UIST21}, which contains $\approx$24k  UI screens (with screenshots, UI hierarchies, and metadata) for $\approx$6.4 Android apps of different domains. This dataset is a subset of the popular \rico dataset~\cite{rico} and includes only UI screens with \textit{complete} and \textit{accurate} UI screenshots, hierarchies, and metadata.
\looseness=-1


We adopted a multi-step procedure to generate screen/component OBs and associated UI screens/components. From this data, we defined the queries, the ground-truth UI screens/components, and the corpus required for component and screen retrieval. Our procedure was designed to generate realistic OB/bug descriptions from the \ricosca UI screens/components, with the goal of generating a diverse and reasonable dataset that could be used to help the models learn associations between related bug descriptions and UI screens, even though the screens may not display a buggy app behavior. 
\looseness=-1

\subsubsection{\textbf{Synthetic OB Generation}}

To generate OBs, we designed bug description templates for a variety of mobile app bug types~\cite{Escobar:TSE20} and specific UI component types. The templates were designed based on discourse patterns that prior work derived from real-life bug descriptions~\cite{Chaparro2017-2}. We designed and implemented heuristics to extract the information from applicable UI screens/components and fill in the templates. These heuristics were executed to generate bug descriptions. This process was iterative and included manual validation of the templates and generated OBs, which resulted in template and heuristic refinement to maximize data quality. Similar procedures have been adopted to generate synthetic UI-level actions in the context of command-UI grounding~\cite{bai2021uibert}. 

\Cref{tab:ob_templates} provides examples of the OB templates we designed and the OB descriptions the templates generate. Each template was created based on one or more discourse patterns and is applicable to one bug type and different kinds of UI components. For space reasons, we provide examples of these elements, but the full catalog of templates (and their implementation) can be found in our replication package \cite{package}.


We now provide details about our OB generation procedure.
\underline{Selecting Bug Types.} Based on the mobile app bug taxonomy from Escobar \etal~\cite{Escobar:TSE20} and a manual analysis of bug reports, we selected nine (9) bug types that cover a variety of app problems, including crashes,  cosmetic issues, and incorrect GUI behavior. Specifically, we selected seven UI bug types from Escobar \etal's taxonomy~\cite{Escobar:TSE20} (\eg \textit{Component with wrong dimensions} and \textit{Wrong text in component} -- see \Cref{tab:ob_templates}), which was derived from manual analysis of Android app bug reports, bug-fixing commits, technical forum discussions, Android documentation, prior bug taxonomies, and online app reviews. Additionally, we selected two additional UI bug types (\ie \textit{Unclickable/uneditable components}), not found in Escobar \etal's taxonomy, by analyzing the titles of sampled bug reports we collected to guide the design of component/screen OB templates (more details below).


\underline{Selecting Applicable UI Components.} Next, we identified the UI components that (1) could be affected by the bug types, and (2) contained potentially useful information to generate OB templates. For example, \textit{Uneditable component} bugs are exclusive to EditText components (\ie text fields). Another example is a bug about \textit{Elements not listed in the right order}, which refers to sets of UI components displayed in the wrong order. Since these are bugs that affect regions of the screen (\ie they would correspond to screen OBs), we identified component containers such as ListView and ScrollView as potentially useful to define proper templates and the screens these templates apply to.

\underline{Assigning Discourse Patterns to Bug Types.}  Prior work identified 90 discourse/linguistic patterns that bug reporters recurrently use to express OB/bug descriptions~\cite{Chaparro2017-2}, based on the manual analysis of $\approx$3k bug reports from nine software projects (including one Android app). Of these 90 patterns, 12 are commonly used by reporters and were found in $\approx$83\% of the 3k reports. We assigned subsets of these 12 patterns to one or more bug types when applicable. For example, \textit{incorrect text} bugs can be expressed using the discourse pattern NEG\_AUX\_VERB, which refers to OB  sentences containing auxiliary verbs that convey a negative discourse (\eg ``I cannot zoom in on the filter screen'').



\underline{Defining OB Templates.} For each bug type, we generated one or more templates applicable to corresponding UI components or screens, by creating a phrase that followed a discourse pattern. An OB template contains: (1) \textit{slots} that represent either components or screens (noted with squared brackets in \cref{tab:ob_templates}), and are filled in from UI screen/component metadata, (2) \textit{variable phrases} are expressions that can be substituted with synonyms to increase OB diversity (noted with braces in \cref{tab:ob_templates}), and (3) \textit{fixed phrases} are expressions that connect \textit{slots} and \textit{variable phrases}. An example of a template for \textit{incorrect dimension} bugs is ``[component] \{dimension\} is \{wrong\}'', where [component] is the slot that represents a UI component expression and \{dimension\} and \{wrong\} are variable phrases that can be used as is or replaced with synonyms such as \textit{size} and \textit{incorrect}, respectively.

Since we initially struggled to define screen OB templates, we guided our template design based on a manual analysis of Android app bug reports. From the original 6,356 bug reports mined by Wendland \etal~\cite{wendland2021andror2}, from which the AndroR2 dataset was built, we took a representative random sample of reports (362 in total at a 95\% confidence level), analyzed their titles, and found that 59 titles describe screen-related bugs (\ie those affecting the entire screen or regions of it). From these titles, we designed screen OB templates, after we identified the corresponding discourse patterns from Chaparro \etal~\cite{Chaparro2017-2}. 

Since screen OBs are more general than component OBs, as they refer to app features or screen-level app behavior rather than specific components, we designed the screen OB templates for screens with certain characteristics rather than templates applicable to every screen in our dataset. With this strategy, we also aimed to help the models learn better the associations between the OBs and screen characteristics. For example, the S2 template in \cref{tab:ob_templates} refers to updates that should happen in settings screens (identified by a search for keywords such as \textit{settings} or \textit{configuration} in the screen/component metadata).



In total, we designed 38 templates, 21 for generating component OBs, and 17 for generating screen OBs.


\begin{table*}[t]
	\caption{Statistics of the synthetic dataset of OB/bug descriptions}
	\label{tab:synthetic_data_stats}
	\setlength\tabcolsep{2.5pt}
	\begin{adjustbox}{width=\textwidth}
		\begin{tabular}{l|cr|cr|ccr|ccr|ccr}
			\toprule
			& \multicolumn{2}{c|}{\textbf{\# of UI screens}}             & \multicolumn{2}{c|}{\textbf{\# of UI components}} & \multicolumn{3}{c|}{\textbf{\# of Component OBs}}                 & \multicolumn{3}{c|}{\textbf{\# of Screen OBs}}                 & \multicolumn{3}{c}{\textbf{\# of Components \& Screen OBs}}             \\ \hline
			& \textbf{Per app} & \cellcolor[HTML]{FFFFFF}\textbf{Total} & \textbf{Per screen}       & \textbf{Total}        & \textbf{Per app} & \textbf{Per screen} & \textbf{Total}     & \textbf{Per app} & \textbf{Per screen} & \textbf{Total}  & \textbf{Per app} & \textbf{Per screen} & \textbf{Total}     \\ \hline
			\textbf{Training}      & 3.6 (2)          & 15,268                                 & 12.4 (10)                 & 189,612               & 416.4 (222)    & 115.5 (85)          & 1,751,224          & 20.7 (12)        & 7.1 (6)             & 61,631          & 252.4 (66)       & 76.0 (37)           & 1,812,855          \\ \hline
			\textbf{Validation} & 3.8 (2)          & 3,685                                  & 12.5 (9)                  & 45,915                & 429.6 (226)      & 114.2 (84)          & 417,538            & 22.2 (13)        & 7.1 (6)             & 15,747          & 257.9 (64)       & 73.8 (35)           & 433,285            \\ \hline
			\textbf{Testing}       & 3.9 (3)          & 4,949                                  & 12.6 (10)                 & 62,444                & 449.6 (241)      & 116.1 (85)          & 570,953            & 22.3 (13)        & 7.1 (6)             & 20,749          & 269.1 (65)       & 75.5 (73)           & 591,702            \\ \hline
			\textbf{Total}      &     \textbf{3.7 (45)}             & \textbf{23,902}                        &    \textbf{12.5 (10)}                       & \textbf{297,971}      &    \textbf{424.9 (226)}              &       \textbf{115.4 (85)}              & \textbf{2,739,715} &  \textbf{21.3 (13)}                &       \textbf{7.1 (6)}              & \textbf{98,127} &    \textbf{256.5 (65)}              &      \textbf{75.6 (37)}               & \textbf{2,837,842} \\ 
			\bottomrule
			\multicolumn{14}{c}{\scriptsize Per app/screen numbers are average values (median values in parenthesis)}  \\ 
		\end{tabular}
	\end{adjustbox}
 \vspace{-0.6cm}
\end{table*}



\underline{Designing Heuristics.} We defined a predefined set of phrases to fill in the \textit{variable phrases}, by selecting one phrase randomly every time the template was applied. 

To fill in template \textit{slots}, we defined rules to compose phrases corresponding to components and screens. These rules would select UI component metadata, particularly, the component text (\ie label), ID, description, type, and location, if/when available. For components, we selected the first available attribute among the text, description, and ID (in that order), as the component phrase for the slot. To increase diversity, we randomly appended the component type and/or the component location on the screen (based on their coordinates and size). For example, for a text field with attributes (text: null, description: ``SSID", ID=null, type=``EditText'') possible created component phrases are \textit{SSID}, \textit{SSID text field},  \textit{SSID text field at the top left corner}, or  \textit{SSID at the top left corner}. Similar rules were defined for generating screen phrases (\ie extract screen names from pre-processed activity names).



\underline{Generating OB Descriptions.}
The defined heuristics were implemented via algorithms that applied the templates on the $\approx$24k UI screens. Only the visible UI components that are leaf nodes in the UI hierarchy were processed to generate OB descriptions, as we consider them as common candidates for reporters to include in their bug descriptions. The algorithms generated unique OBs and avoided cases where the OBs were excessively long (\eg from long component metadata).

In total, we generated $\approx$2.8M OB descriptions (75.6/256.5 per screen/app on average)---see \cref{tab:synthetic_data_stats}. From these, $\approx$2.7M are component OBs (115.4/424.9 per screen/app on average) and $\approx$98k are screen OBs (7.1/21.3 per screen/app on average). 

\underline{OB Template/Heuristic Validation and Refinement.} The templates, heuristics, and generated OBs were validated in multiple review sessions where a sample of OBs, generated by different templates, was manually inspected by two or more authors. The authors reviewed grammar, semantics, and how realistic the bug descriptions were, suggesting adaptations to improve the templates and heuristics.







\begin{table*}[t]
	\caption{Examples of templates used to generate synthetic OB/bug descriptions} 
	\centering
	\label{tab:ob_templates}
	\scriptsize
 \setlength{\tabcolsep}{4pt}
	\begin{adjustbox}{width=\textwidth}
	\begin{tabular}{M{0.11\textwidth}|M{0.24\textwidth}|M{0.3\textwidth}|M{0.121\textwidth}|M{0.13\textwidth}}
\toprule
\textbf{Bug Type~\cite{Escobar:TSE20}} & \textbf{Template}                                                 & \textbf{Generated OB (App name)}                                                      & \textbf{Screens/Components}   & \textbf{Discourse Pattern~\cite{Chaparro2017-2}} \\ \midrule
\multicolumn{5}{c}{\textbf{Templates for Screen OBs}}  \\ \midrule
Elements not listed in the right order & \textbf{S1}: After \{filtering\} the {[}list{]}, the order of {[}list item{]} did not change & After filtering the view items list, the order of new cars did not change (Autoportal) & Screens with ListViews, ScrollViews, etc. & AFTER\_NEG                 \\ \hline
UI refresh issue                       & \textbf{S2}: \{Changes\} in the {[}screen{]} setting \{will not apply immediately\}          & Changes in the app settings will not apply immediately (smartChord)                    & Settings screen                           & NEG\_AUX\_VERB             \\ \hline
Issues in view animation               & \textbf{S3}: I cannot \{zoom on\} the {[}screen{]}                                          & I cannot pinch on the home wiki screen (FANDOM)                                        & All screens                               & NEG\_AUX\_VERB             \\ \midrule

\multicolumn{5}{c}{\textbf{Templates for Component OBs}} \\ \midrule
Component with wrong dimensions & \textbf{C1}: {[}Component{]} \{size\} does not \{match the expected size\} & The More options button does not match the expected size (Daily Reflections) & All components & NEG\_AUX\_VERB             \\ \hline
Wrong text in component & \textbf{C2}: \{Wrong\} text in {[}component{]} & Incomplete text in Invite your friends textview (Chat Rooms) & Buttons, TextViews, etc. & VERB\_TO\_BE\_NEG          \\ \hline
Unsupported style in component & \textbf{C3}: {[}Component{]} \{shows\} \{incorrect\} \{color\} & ECONOMY button shows incorrect text color when clicked (PlayCast) & Radio buttons, TextViews, etc. & NEG\_ADV\_ADJ              

\\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-0.5cm}
\end{table*}






\subsubsection{\textbf{Synthetic Retrieval Data}} 

We kept track of the UI screen used to generate each screen OB and the UI screen/components used to generate each component OB. Based on this information, we defined the queries, ground truth, and corpus for both screen (SR) and component retrieval (CR). 

For SR, the queries are \textit{both} component and screen OBs ($\approx$2.8M total), the ground truth is their corresponding UI screen (one per query), and the retrieval corpus comprises the screens that belong to a specific app (there are 3.7 screens per app, on average). SR retrieval is performed per app (\ie rather than across apps), as it would be executed in practice.
\looseness=-1

For CR, the queries are only component OBs ($\approx$2.7M total), the ground truth is their corresponding UI component (one per query), and the retrieval corpus is the UI components for a given screen (there are 12.5 components per screen, on average).
\looseness=-1







\subsection{Real Dataset Construction}
\label{subsec:real_data}

We built a real-life dataset of bug descriptions and relevant UI screens/components to assess the effectiveness of the models in a realistic setting. 


\subsubsection{\textbf{Bug Report Selection}}

We leveraged the AndroR2 dataset~\cite{wendland2021andror2, Johnson2022AndroR2+} to select the bug reports for our study. This dataset consists of 180 manually reproduced bug reports for popular open-source Android applications hosted on GitHub. These reports were systematically collected from the project's issue tracker following a rigorous procedure (see \cite{wendland2021andror2, Johnson2022AndroR2+} for details). The dataset provides APK files, buggy and bug-fixing commits, GitHub issue links, and scripts that replicate the reported bugs (crash-, output-, navigation-, and cosmetic-related bugs~\cite{wendland2021andror2, Johnson2022AndroR2+}).
\looseness=-1

From these 180, we selected a subset of 53 bug reports, which are included in a recently-constructed dataset by our research lab to conduct research on automated bug localization in Java source code. Our research lab conducted a rigorous manual procedure to collect ground-truth buggy Java files for the 180 AndroR2 reports. Multiple lab members (including some of the authors of this paper) reproduced the reported bugs in a Pixel 2 Android emulator and for the reproducible bugs, they inspected the bug-fixing commits to identify the Java files and lines of code that were changed to fix the reported bug.  From the 180, 100 reports were discarded because: (1) their bugs are not reproducible, (2) included fixed non-Java files only, (3) are no longer publicly available, or (4) included ambiguous code changes or commit IDs. From the 80 remaining reports, we selected the first 53 to be used in our study. 

From the 53 bug reports (1 to 6 per app), 17 describe an output problem, 15 reports an app crash,  14 describe a UI cosmetic issue, and 7 report a navigation problem. The bug reports correspond to 29 Android apps (\eg GnuCash~\cite{GNU}, Mozilla Focus~\cite{bugzilla}, K-9 Mail~\cite{K-9}, WiFi Analyzer~\cite{wifianalyzerbug}, Images to PDF~\cite{Images2PDF}) of different domains (\eg  finance tracking, web browsing,  emailing, WiFi network diagnosis, and image conversion) and UI layouts.


\subsubsection{\textbf{Bug Description Annotation}}

To collect bug descriptions, two authors inspected and annotated the OB sentences in the title and descriptions of the 53 bug reports. Based on the definition of OB and the criteria to annotate OB sentences defined by Chaparro \etal~\cite{Chaparro2017-2}, one author marked every sentence of the bug reports that conveyed a bug manifesting in the UI. The second author verified the first author's annotations, marking missed OB sentences and incorrect annotations, resulting in an agreement for 1774/1807 ($\approx$98\%) sentences (Cohen's kappa \cite{Cohen} of 0.91). The authors solved disagreements via discussion and consensus. Reasons for disagreement included mostly mistakes and misinterpretations (\eg when sentences described root causes in the code, rather than UI faults). In total 127 sentences were identified as OB/bug descriptions, which represent the queries for retrieval.

\subsubsection{\textbf{Retrieval Corpus Collection}}

To build the retrieval corpus for each bug description, we require the set of UI screens/components of the apps, including the buggy ones. To collect these data, we employed: (1) a record-and-replay methodology used in prior studies~\cite{Cooper:ICSE21,song_toward_2022}, and (1) an automated app exploration methodology used by Chaparro \etal~\cite{Chaparro:FSE19}.
\looseness=-1

The goal of the record-and-replay methodology was to collect the buggy UI screens for each bug report and the UI screens navigated while reproducing the bugs. Two authors manually reproduced the reported bugs by executing the reproduction steps from the bug report on a Pixel 2 Android emulator.
While reproducing the bugs, the authors used the AVT tool~\cite{Cooper:ICSE21,song_toward_2022} to collect UI-event traces and a video showing the user interactions of the app and the bug \cite{Moran:2017, Moran2016}. These traces were replayed on the emulator via the TraceReplayer tool, which is able to collect app screenshots and UI hierarchies/metadata for the exercised app UI screens.
\looseness=-1

The purpose of the automated app exploration methodology was to collect as many UI screens for building the corpus. We executed a version of the \crashscope tool~\cite{Moran:2017} that implements multiple exploration strategies to interact with the UI components of app screens in a comprehensive way, trying to exercise as many screens as possible. In the process, \crashscope collects app screenshots and XML-based UI hierarchies/metadata for the exercised app UI screens.

Since these two approaches can generate duplicate UI screens, we employed the approach by Chaparro~\etal~\cite{Chaparro:FSE19} to produce a unique set of UI screens for each of the 53 bug reports. This approach parses the hierarchies of the collected UI screens for an app and establishes uniqueness between two screens if they have the same hierarchical structure (based on component types, sizes, and parent-children relationships). This implies that two UI screens with the same structure but different text shown on the screen are considered the same.

This procedure resulted in UI screen corpora containing $\approx$29 UI screens per query on average.



\subsubsection{\textbf{Ground Truth Construction}} 

During three annotation sessions, three authors (\aka annotators) first read and understood the reported bugs, watching (if needed) the bug reproduction video collected during the corpus collection step.  
Then, the annotators inspected the app screens from the corpus to identify the buggy screens shown in the video and marked them properly in a spreadsheet (with unique identifiers). The annotators then identified the OB type of the bug descriptions, as either screen or component OB, according to the definition given in \cref{sec:problem_motivation}. For component OBs, the annotators identified and marked the buggy components in the same spreadsheet. This process included discussion among the annotators, and reaching a consensus when disagreements happened.

The annotators rated the quality of the bug descriptions based on the amount of information they provided to understand what the bug report is about. Since the OB-UI retrieval tasks focus on individual bug descriptions, the annotators judged the quality of single OBs in isolation. The annotations agreed on a quality rating on a 1-5 scale. A rating of 1 means the bug description does not contain useful information to understand the problem. Conversely, a rating of 5 means the description contains complete information to understand the bug. A rating of between 1 to 5 indicates that there is missing information in the OB that hinders bug comprehension. 


\subsubsection{\textbf{Real Retrieval Data}} 
For SR, the queries are both component and screen OBs (127 total---see \cref{tab:real_data_stats}) with 1.7 buggy UI screens on avg. as ground truth and 29.3  screens in the corpus on avg.

For CR, the queries are created from component OBs. Since these OBs may be associated with multiple buggy screens, each screen represents a retrieval task. This means we created 89 queries (or retrieval tasks), with 4.3  buggy UI components on avg. as ground truth and 28.1 components in the corpus on avg.
\looseness=-1

\begin{table}[t]
	\caption{Statistics of the real data for screen/comp. retrieval}
	\label{tab:real_data_stats}
	\setlength{\tabcolsep}{2pt}
	\begin{adjustbox}{width=\columnwidth}
	\begin{tabular}{l | c | ccc}
		
		\toprule
		& \multicolumn{1}{c|}{\textbf{Comp. Retrieval}} & \multicolumn{3}{c}{\textbf{Screen Retrieval}}                        \\ \hline
		\textbf{Statistic \textbackslash OB Type}           
		          & \textbf{Component}                            & \textbf{Screen} & \textbf{Comp.} & \textbf{Src. \& Comp.} \\ \hline
		\textbf{\# of OBs}       & 54                             & 73       & 54          & 127                 \\ \hline
		\textbf{\# of retrieval tasks}          & 89                                            & 73              & 54                 & 127                         \\ \hline
		\textbf{OB length (words)}        & 11.5 (9)                                      & 11.2 (9)        & 11.1 (9)           & 11.1 (9)                    \\ \hline
		\textbf{\# of buggy elements}   & 4.3 (3)                                       & 1.7 (1)         & 1.7 (1)            & 1.7 (1)                     \\ \hline
		\textbf{Corpus size} & 28.1 (18)                                     & 26.9 (22)       & 32.5 (24.5)        & 29.3 (24)                   \\ 
		\bottomrule
		
		\multicolumn{5}{c}{\scriptsize Average (median) values per query/retrieval task}  \\ 
	\end{tabular}
\end{adjustbox}
\vspace{-0.6cm}
\end{table}












\subsection{Model Fine-tuning and Execution}
\label{subsec:eval_settings}




We split the $\approx$6.4K apps in our synthetic dataset into training (65\%), validation (15\%), and test sets (20\%). The training set (\ie the OBs and their ground truth for the training apps) was used for fine-tuning the models, the validation set was used for hyper-parameter tuning, and the test set for assessing model performance. We denote the fine-tuned models by their name followed by the $ft$ subscript; for example, we denote fine-tuned \clip as \clipf.

For fine-tuning \textbf{\sbert}, we required building sets of positive and negative pairs of OB descriptions and textual documents of UI screens/components. UI component documents were defined by concatenating the component text, description, and ID. UI screen documents were defined by concatenating the UI component documents. We experimented with different strategies for building positive and negative pairs, but the one that led to the highest performance was the following. Half of the training OBs and their corresponding UI screen/components were used as positive pairs and the remaining half of OBs were used to create negative pairs. To create these pairs we randomly selected screens from other apps (for SR), or other components from the screen (for CR). Our replication package describes the other data creation strategies we experimented with and the respective results~\cite{package}.


For fine-tuning \textbf{\clip}, we required pairs of OB descriptions and images of the ground-truth UI screens/components.  We experimented with different datasets created from the training set. Using the entire training set for fine-tuning proved to be ineffective since a single UI screen/component can have multiple OBs associated with it, which makes it difficult for \clip  to learn the distinction between different pairs containing the same image (given its contrastive architecture). We experimented by using subsets of 1, 5, 10, and 15 OBs per image (selected from different bug types), all leading to better performance on the synthetic test set. In the end, the best performance was obtained by using unique pairs of OBs and images (\ie one OB per image), preserving the distribution of component/screen OBs of the training data, and using OBs of different bug types across different images. The performance on this data can be explained by \clip's contrastive architecture.

Fine-tuning \textbf{\blip} requires the same information sources as \clip. Given \blip's similarity to \clip regarding architecture, we experimented with the same subsets of pairs and the unique pairs of OBs and images as used for \clip.

Once fine-tuned, the models were tested on the synthetic test set as well as on the real dataset. \textbf{\lucene}, being an unsupervised approach, was only tested on the aforementioned data, following the same procedure as for \sbert to create textual documents from UI screens/components. Only for \lucene, we performed standard pre-processing on the queries and documents  (lemmatization, stop word removal, \etc).






\subsection{Bug Localization Experiments Execution}
\label{subsec:bl_methodology}
For validating the usefulness of OB-UI mapping tasks, we leverage the retrieved screens from SR to automate a SOTA bug localization (BL) approach \re. The BL approach (we will refer to it as manual BL) \re requires the interaction traces (buggy screen information) of the bug reproduction to boost, filter, query reformulation, and query expansion to improve the performance. The interaction trace collection process is fully manual which is both laborious and time-consuming. As the SR of OB-UI mapping can identify the buggy screens, we hypothesized that we could leverage this information for bug localization and automate bug localization (we will refer to it as automatic BL).

One difference between the OB-UI mapping and bug localization is the query. While the query for the bug localization is the whole bug report text, the query for the mapping is only the OB sentence. As a result, there can be multiple OB sentences for the same bug report for mapping. To deal with this situation, we derived SR results in two mapping settings: (1) Concatenated OBs: all OBs of a bug report is concatenated to form a single query for each bug report, and (2) First OB: the first OB (71 out of 79 OBs are found in the title) is taken as the query from each bug report. We utilized the SR results of the best mapping model (\ie \ \blip) for conducting BL experiments. Note that we used 79 bug reports out of 80 bug reports of the BL dataset (one bug report is excluded as it was not reproduced).

Among the models explored in the BL approach \re, we decided to run experiments on the LUCENE and BugLocator models. We conducted extensive experiments on all the feasible BL configurations in two settings: (1) 3 Screens: top 3 retrieved screens of SR is used as the bug state for BL, and (2) 4 Screens: top 4 retrieved screens of SR is used as the bug state for BL. These 3 settings are executed for both the mapping settings resulting in 12 experiments in total for the 2 models (xxxx total configurations) \antu{Update this.}. Note that for 4 Screens experiments, we used 77 bug reports as 2 bug reports have only 3 retrieved screens. All the BL experiments are the same as the proposed approach \re, except that instead of manually collected GUI information, we utilized the GUI information retrieved from the SR task of OB-UI mapping. 



\subsection{Evaluation Metrics}
\label{subsec:metrics}



We used standard retrieval metrics, widely used in prior studies~\cite{akbar2020large,lee2018bench4bl,florez2021combining,Cooper:ICSE21}, to measure the effectiveness of the models. We used \textbf{MRR}, \textbf{MAP}, and \textbf{HIT@K} (a higher value indicates a better model performance).
\textbf{Mean Reciprocal Rank (MRR)} is the average of the \textit{reciprocal ranks} (\ie $\frac{1}{rank}$)  computed for a set of queries, where $rank$ is the position of the first buggy UI screen/component retrieved by an engine for a query.  \textbf{Mean Average Precision (MAP)} measures the effectiveness of a retrieval engine by calculating the mean of the \textit{average precisions} of a set of queries. The average precision measures the average number of buggy UI screens/components retrieved at different cut points of the result list. \textbf{HIT@K} (or \textbf{H@K}) is the proportion of queries for which an engine can retrieve the expected buggy UI screen/documents in the top-K results. While MRR and MAP consider the entire list of the retrieved elements, H@K considers the top-K retrieved results.


























